On Liveness of Dynamic Storage

Dynamic distributed storage algorithms such as DynaStore, Reconfigurable Paxos, RAMBO, and RDS, do not ensure liveness (wait-freedom) in asynchronous runs with infinitely many reconfigurations. We prove that this is inherent for asynchronous dynamic storage algorithms, including ones that use $\Omega$ or $\diamond S$ oracles. Our result holds even if only one process may fail, provided that machines that were successfully removed from the system's configuration may be switched off by an administrator. Intuitively, the impossibility relies on the fact that a correct process can be suspected to have failed at any time, i.e., its failure is indistinguishable to other processes from slow delivery of its messages, and so the system should be able to reconfigure without waiting for this process to complete its pending operations. To circumvent this result, we define a dynamic eventually perfect failure detector, and present an algorithm that uses it to emulate wait-free dynamic atomic storage (with no restrictions on reconfiguration rate). Together, our results thus draw a sharp line between oracles like $\Omega$ and $\diamond S$, which allow some correct process to continue to be suspected forever, and a dynamic eventually perfect one, which does not.

==> sections/abstract.tex <==
\section{Abstract}
TBD

==> sections/contribution.tex <==


\section{Contributions and previous work}

In this work we try
to illuminate the subtle differences among asynchronous
systems that compute with infinitely many processes,
particularly models $M_2,M_3,D_2$ and $D_3$ in message passing
and shared memory systems. We ask what can and what cannot be
constructing atomically and in a wait-free manner in these
models.
To be precise, we are interested in what models we can
simulate a MWMR register, as well as counter and snapshot
objects, assuming communication via shared memory, and in what
dynamic models we can simulate a MWMR register assuming message
passing communication.

\subsection{Shared memory}

In Section \ref{sec:mutable}, we generalize
Aguilera's~\cite{aguilera2004column} unproven claim regarding
the impossibility of emulation of MWMR registers from SWMR ones
in $M_2$ and $M_3$. We extand this result to a class of objects
we call \emph{mutable} as defined in Section \ref{sec:mutable}.

In order to circumvent this impossibility, we move to dynamics
models.
In Section \ref{sec:snap} we present an algorithm that
solves the dynamic snapshot problem in $D_3$ via shared
memory communication, and assumes SWMR registers only.
From this algorithm, in turn, a MWMR register, a counter and
other mutable objects can be simulated as we also show therein.
This result demonstrates the subtle differences among the models
and shows that $D_3$ is strictly stronger than $M_3$ and $D_2$
is strictly stronger than $M_2$ in shared memory systems.
Although they all allow participating of infinitely many
processes, most interesting objects that cannot be realized
in $M_2$ assuming SWMR registers, can be implemented in $D_3$.

Gafni et al. \cite{gafni2001concurrency} introduced the
\textit{bounded-snapshot} problem, and showed that it is
solvable in $M_2$ but not in $M_3$, in order to prove that $M_3$
is less powerful than $M_2$. It is easy to show that this
problem is also not solvable in $D_3$, and therefore, together
with the solvability of dynamic snapshot problem, we conclude
that $M_2$ and $D_3$ are incomparable.

\subsection{Message passing}

A natural question arises about message passing
systems: can we simulate a dynamic MWMR register in dynamic
models. Notice that without oracle that helps new arrival
processes to find an added and not removed process, models $M_2$
and $M_3$ make no sense in message passing systems.

There were many works in the last decade that deal with
%emulation of atomic storage via message passing in
%reconfigurable systems.
this question. 
Some of them use the quorum based
approach~\cite{ShraerDynadisc,lynch2002rambo,dynastore,gilbert2003rambo,gilbert2010rambo}
,while others rely on state machine replication
(SMR)~\cite{SMRlamport2010reconfiguring,SMRvirtually}.
Aguilera et al.~\cite{dynastore} assumed a fully asynchronous
model and presented DynaStore, which
simulates an atomic MWMR register in $D_2$ via message passing
communication under assumptions on failure patterns that
generalize the correct majority criterion to a dynamic model.
Lynch et al. presented RAMBO~\cite{lynch2002rambo}, which uses
consensus to agree on reconfigurations, while read and write
operations are asynchronous,
whereas~\cite{SMRlamport2010reconfiguring,SMRvirtually}
described how to reconfigure state machine replication, and in
turn use it to implement dynamic atomic storage.

To the best of our knowledge none of the previous work, whether
assuming a fully asynchronous model or using consensus,
presented an algorithm that ensures completion of active-forever  
process's operation in the presence of endless reconfigurations
(model $D_3$).

Consider some leader based algorithm and a scenario with endless
reconfigurations. The leader may always be changed due to a
removal of previous leader. In this case it is possible that a
slow active-forever process is never able to communicate with
any leader, and therefore its operation never completes.

In Section \ref{sec:imposStorage}, we show that it is inherent,
and there is no emulation of atomic
shared storage in message passing model $D_3$ even if the
processes can solve consensus in every configuration.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
Aguilera et al.~\cite{dynastore} presented DynaStore, which
simulates an atomic MWMR register in $D_2$ via message passing
communication under assumptions on failure paterns that
generalize the correct majority criterion to a dynamic model.

Yet the existence of such an algorithm in $D_3$ remained an open
question.

In Section \ref{sec:imposStorage}, we answer this
question by proving that there is no emulation of shared storage
in message passing model $D_3$.
\end{comment}
%
\begin{center}
	\begin{table}[H]
	\label{table:questions}
    \begin{tabular}{ | p{3cm} | p{3cm} || p{4.0cm} | p{4.6cm} | }
    \hline
    Communication & Concurrency  & MWMR register & Snapshot and counter
     \\ \hhline{|=|=|=|=|}
    Shared memory, MWMR regs. & $M_2$ or $M_3$ & Yes (given)
    & Yes~\cite{gafni2001concurrency} \\ \hline 
    Shared memory, SWMR regs. & $M_2$ or $M_3$ & No,
    claimed by~\cite{aguilera2004column},  proven in Section
    \ref{sec:mutable}  & No,  Section
    \ref{sec:mutable}
    \\
    \hline Shared memory, SWMR regs. & $DM_2$ or $DM_3$ &
    Yes,  Section \ref{sec:snap}.
     & Yes, Section \ref{sec:snap}  \\ \hline 
    Message passing & $DM_2$ & Yes, dynaStore~\cite{dynastore} &  
    \\
    \hline
    Message passing & $DM_3$ & No, Section
    \ref{sec:imposStorage} &   \\
    \cline{3-4} &&  Possible with oracle, Section
    \ref{sec:diamondP} & 
    \\
    \hline
    \end{tabular}
    \caption{Summary of results.}
	\label{table:table2}
    \end{table}
\end{center}
%
An interesting question that rises from the impossibility
result is whether this problem is solvable with stronger oracle.
In Section \ref{sec:diamondP}, we define a dynamic version of
the eventually perfect failure detector $\diamond
P$~\cite{aguilera2001stable}, which we call $\diamond P^D$, and
implement helping mechanism to circumvent the impossibility
result. We present an algorithm, based on state machine
replication, that emulates an atomic dynamic MWMR resister
under DynaStore failure model in $D_3$ via message passing. 
Unlike static failure
detectors, $\diamond P^D$ is queried regarding the liveness of
processes, separately for each process, and it returns for each
queried process ``ok'' or ``fail''.
For each process, it can return incorrect answers,
but it eventually returns only correct ones. 

\begin{comment}
This failure detector is quite strong, and in static systems
weaker failure detectors exist~\cite{Chandra}. For example, the
stable leader oracle $\Omega$ is known to be the weakest failure
detector to solve consensus~\cite{chandra1996weakest}. However,
it is unclear how the definition of $\Omega$ can be transformed
to a dynamic model. Indeed, in such models every process can be
removed from the $current$ set, so it is impossible to guarantee
a stable leader.

The question whether there is a weaker failure detector that can
be used to solve this problem in $D_3$ is remains open.
\end{comment}

The summary of our results is presented in Table
\ref{table:table2}.




==> sections/diampndPOldAlg.tex <==
 
\subsection{Dynamic Storage}
\label{sub:oracleAlg}

%TODO: exlain write and read again.. I added phase..

Previous implementation of reconfigurable SMR does not guarantee
termination of slow process's operations. Consider scenario in
which there is a presence of endless reconfigurations, in this
case the leader may always change, and slow process that is
always in the minority will never be able to communicate with
the leader.

In order to solve the problem we use $\Diamond P^D$. Process
$p_i$ that wishes to perform an operation first send 
to every process in the latest configuration its log, and wait
for reply from every non suspicion process. In each reply from
process $p_j$, $p_j$ tells $p_i$ what the operation that it
currently tries to perform.  



Our algorithm uses $\Diamond P^D$ in order to  a SMR approach
combi 


The algorithm uses consensus in order to agree on the order of
the configurations, and quorum-based operations to ensure
atomicity.
We assure the liveness properties by using a helping
mechanism.




\begin{definition}

We say that a configuration $c$ is $stable$ if it is either
the initial configuration or some process completes line 12 in
$TwoPhaseUpdate(c)$ procedure. In other words, a majority of the
previous configuration receives $c$ and the value that is stored
in the previous configuration is written to $c$.

If a configuration is not $stable$, then we call it $pending$.
We say that a new configuration is generated when the consensus
procedure returns new TS. In other words, when some process win
a consensus object.

\end{definition}


Every configuration is associated to a different consensus
object. We assume $consensus$ procedure, which is called by
every process that wish to change the configuration. The
procedure gets a configuration $c$ and a finite set of changes
$Cng \in Changes$ .
If $Cng$ has been already chosen before (in one of the previous
objects), then the procedure returns $\perp$. Otherwise It
returns the changes that were chosen in the consensus object
corresponding to c with its time stamp, and a pointer to the
next object (New time stamp for every object).
Notice that in this way we have total order on the
configurations. We denote the configuration with the highest
time stamp at any moment to be $new$ and the one before it to be
$old$. Notice also that a finite known set of processes
participate in each consensus object (the members of the
associated configuration), so the consensus can be solved by
using $\Diamond P^d$ failure detector. 

The main key in the algorithm is that process that wishes to
change the $new$ configuration must first help to all other
process that the failure detector thinks is correct. 
The failure detector is eventually perfect, thus every correct
slow process eventually receives help.
 
Every process $p$ has two local registers, $r$ and $Op$. Where
$Op$ holds information about $p$'s current operation. And $r$
holds information about the system. Register $r$ has four fields: 
$value$, $ts_v$, $current$, and $pending$. Where $value$ is the
most updated value that $p$ got and $ts_v$ is the corresponding
time stamp. $current$ and $pending$ are configuration
represented by a tuple, which consist of a set $mem$ of
processes belonging to the configuration, a pointer $pointer$ to
its consensus object, and a time stamp $ts$.

Every process $p_i$ stores in $r_i.current$ the most updated
stable (not pending) configuration, and in $r_i.pending$ the
most updated pending configuration it knows about. Notice that
the value that a process stores is not necessarily as updated as
the configuration its stores. However, this is not a problem since
the value and the configurations have different time stamps, and
the algorithm guarantees that a $new$ configuration becomes
stable only after a majority of its members receives the value
that is stored in the $old$ (previous) configuration.  

Important to notice that in this algorithm we allow only one
concurrent pending configuration. Process that performs
reconfig operation must first complete the reconfig of the $new$
configuration. We say that a $new$ configuration stops to be
pending, when both, a majority of $old$ configuration receives
it, and a majority of it receives the value that is written in
$old$ configuration.  
  
In model $D_3$, where infinitely many process may be added,
atomicity is not trivial. We achieve it by $TwoPhaseUpdate$
mechanism. Process $p_i$ that wish to change configuration,
after it wins the appropriate consensus, first sends the $new$
configuration to all the processes in the $old$
configuration (and wait for majority to replay), then it reads
the value from the $old$ configuration and writes it back to
the $new$. Now the $new$ configuration is stable (not pending)
and $p_i$ sends it again to all the processes. Then the
operation returns to the client.

When another process $p_j$ wants to perform $write$ or $read$
operation, it first communicate with the 
$r_j.current$ configuration and then with the 
$r_j.pending$ configuration.
Process that receives WriteRequest or ReadRequest returns also
its current and pending configurations. After receiving replays
from a majority, $p_j$ update its configuration accordingly.
Its operation completes only after no updated configuration
received from the majority, otherwise $p_j$ continue the
operation on the updated configurations.
This way we assure that concurrent readers and writers performs
their operation on the same configurations and therefore readers 
does not miss writes.


%update configuration --> write, write --> update
% configuration

We use helping mechanism to achieve the liveness properties.
process $p$ that wish to change the configuration must first
help to all other correct processes. Recall that in asynchronous
systems process cannot distinguish between slow process and
faulty one, thus we use the $\diamond P_d$ oracle. In the
beginning of a reconfig operation $p_i$ asks all the processes
in $r_i.current$ what operation they are currently perform. Then
for every process, $p_i$ waits for either its replay or for a
notification from the oracle that the process failed.
Before completing the operation $p$ helps all the processes
from which it receives an answer, by completing their writes ,and
reconfig operations, and sending them the read result. The
oracle is eventually perfect, so every process eventually
receives help.

Notice that the oracle helps us to
circumvention the impossibility result, where we use the fact
that process that performs reconfig operation never knows which
processes failed, and therefore the helping mechanism cannot
work.

The data structure is defined in Algorithm~\ref{alg:definitions}

\begin{algorithm}[H]
% \floatname{algorithm}{ALGORITHM:}  
% \renewcommand{\thealgorithm}{}  
 \caption{definitions}  
 \label{alg:definitions}
\begin{algorithmic}

\State $r=\langle value,
ts_v, current, pending \rangle$
\\ \hspace*{1cm}  where $value \in\mathcal{V}\cup \{\perp\}$,
$ts_v \in \mathbb{N}\cup \perp$, \\ \hspace*{1cm} and $current,
pending= \langle mem,removal,ts \rangle$ or $\perp$
\\ \hspace*{2cm} where $mem,removal \subset \Pi$, $ts
\in\mathbb{N}\cup \perp$


\begin{comment}
\State $Op=\langle operation, \langle val, ts \rangle \rangle$
\\ \hspace*{1cm}  where $operation \in
\{\perp,recongig,read,write\}$, $val \in \{ \perp\} \cup
\mathcal{V} \cup 2^\Pi$ \\ \hspace*{1cm} and $ts\in
\mathbb{N}\cup \perp$
\end{comment}

\State $Op= \perp$ or $\langle read \rangle$ or $\langle
write,v,ts \rangle$ or $\langle reconfig, changes \rangle $

\State $P_0\subset \Pi$
\State $configur_0=\langle P_0, pointer, 0 \rangle$
\State $numMsg \in \mathbb{N}$
\State $opMsg \in \mathbb{N}$


\State  $\forall p_i \in \Pi$, $r_i$, $numMsg_i$, $opMsg_i$ and
$Op_i$ are local variables \\ \hspace*{1cm} \textbf{Initially:} $numMsg_i=0$,
$opMsg_i=0$, $Op_i=\perp$, and if $p_i \in P_0$, \\
 \hspace*{4cm} $r_i=\langle \perp,0, configur_0, \perp
 \rangle$ \\ \hspace*{4cm}  else 
$r_i=\langle \perp,0, \perp,\perp \rangle$

\end{algorithmic}
\end{algorithm}

We now describe the Algorithm. We start from $updateCurrent$ and
$updatePending$ procedures, which pseudocode can be found in
Algorithm \ref{alg:update}. Those procedures are called when new
configurations arrived. They assure that $r.current$ holds the 
most updated stable configuration that has been ever received,
and similarly that $r.pendings$ holds the most updated
pending configuration that has been ever received. Notice that
If the
configuration in $r.pendings$ stops to be pending
(the condition in $updateCurrent$ line 3 satisfied), then
$r.pendings$ set to $\perp$.
Notice also that if the condition in line 11 in
$updatePending$ is satisfied, then $r.pending$ is no more
pending and therefore can be written to $r.current$ (line 12).




\begin{algorithm}[H]
% \floatname{algorithm}{ALGORITHM:}  
% \renewcommand{\thealgorithm}{}  
 \caption{Update configurations}  
 \label{alg:update}
\begin{algorithmic}[1]

\Procedure{$updateCurrent$}{$current$}
     \State \textbf{if} $r.pending \neq \perp$ \textbf{then} 
     \State \hspace*{1cm} \textbf{if} $current.ts \geq
     r.pending.ts$ \State \hspace*{1cm} \textbf{then} $r.current
     \leftarrow current$, $r.pending \leftarrow \perp$
     \State \textbf{if} $current.ts>r.current.ts$
     \State \textbf{then} $r.current \leftarrow current$
\EndProcedure

\Statex
\Procedure{$updatePanding$}{$pending$}
   	 \State \textbf{if} $pending \neq \perp$ \textbf{then}	 
     \State \hspace*{1cm} \textbf{if} $pending.ts>r.pending.ts$
     \State \hspace*{1cm} \textbf{then} $r.current \leftarrow
     r.pending$ and $r.pending \leftarrow pending$ 
     \State \hspace*{1cm} \textbf{elseif}
     $pending.ts>r.current.ts$
     \State \hspace*{1cm} \textbf{then} $r.current \leftarrow
     pending$
     
     \State \textbf{elseif} $pending.ts>r.current.ts$
     \State \textbf{then} $r.pending \leftarrow pending$ 
\EndProcedure 


\end{algorithmic}
\end{algorithm}


Operations $read$ and $write$ are presented in  
Algorithm~\ref{alg:ReadWrite}. 
The basic procedures they use are   
$ReadFromConfiguration$ and $WriteToConfiguration$ (lines 1
and 6). Procedure $ReadFromConfiguration$ receives configuration
$cng$, send read request to all the processes in $cng.mem$, and
waits for majority to replay. In similar way Procedure
$WriteToConfiguration$ gets configuration $cng$, $value$, and
$ts$. Sends the $value$ with the $ts$ to all the processes in
$cng.mem$, and waits for majority to replay. Notice that replay
from every process $p_i$ contains $p_i$'s register, and
$r.current$ and $r.pending$ are updated via $updateCurrent$ and
$updatePending$ procedures.

Procedures $RecursiveRead$ (line 11) and $RecursiveWrite$ (line
20) are responsible that the $read$ and $write$ operations will
not complete until they communicate with the $old$ and $new$
configurations. Procedures $RecursiveRead$ receives configuration
$cng$, performs $ReadFromConfiguration(cng)$, and then checks
the configurations $r.current$ and $r.pending$. If they were
updated (during $ReadFromConfiguration(cng)$), then it
recursively call itself with the updated configuration. With
$r.current$ if it was updated, and otherwise with $r.pending$
(this way we ensure communication with $old$ and $new$
configuration). The procedure returns the current value and
time stamp.

Procedures $RecursiveWrite$ is resembling to $RecursiveRead$,
except that it receives also value and time step, uses
$WriteToConfiguration(cng,value,ts)$ instead of\\
$ReadFromConfiguration(cng)$ and does not return any value.

Important to notice that with infinitely many concurrent
reconfig operation those procedures may never return. We solve
this problem with the helping mechanism.

Operation $read$ (line 28), first sets its $Op$ register (line
29). This is part of the helping mechanism, $Op$ is sent to
every process that wants to help. Then it calls to
$RecursiveRead$ with $r.current$, and writes back the read value
via $RecursiveWrite$ starting again from $r.current$
configuration. It is important to start from $r.current$ because
in this way we guarantee that the procedures communicates with
the $new$ and the $old$ configurations. And this is essential in
order to prevent from readers to miss earlier writes.

Operation $write$ (line 36) first set $Op$ to read (instead of
write), because it does not know the time stamp at this point.
Then it performs $RecursiveRead$ to obtain the time stamp. Recall that
$RecursiveRead$ may never return, but in this case some other
process will eventually help. Next it set $Op$ to write, and
invokes $RecursiveWrite$ with $r.current$ (for the same
reasons as in $read$ operation), the desired value and new time 
stamp. This procedure may also never return but again in this
case eventually some other process will help.


\begin{algorithm}[H]
% \floatname{algorithm}{ALGORITHM:}  
% \renewcommand{\thealgorithm}{}  
 \caption{Read $\&$ Write}  
 \label{alg:ReadWrite}
\begin{algorithmic}[1]

\Procedure{$ContactConfiguration$}{$Request,cng,value,ts$}
	\State $M_i \leftarrow \emptyset$
	\State $msgNum_i \leftarrow msgNum_i + 1$
	\State \textbf{if} $Request = readRequest$ \textbf{then}
	\State \hspace*{0.2cm} send $\langle readRequest,
	msgNum_i \rangle$ to all processes in $cng.mem$ 
	\State \hspace*{0.2cm} \textbf{wait} until $\langle Reply,R,
	msgNum_i, \ldots \rangle$ is in $M_i$ from a majority of
	$cng.mem$ 
	\State \hspace*{0.2cm} $t \leftarrow $ maximal time stamp $TS$
	s.t.
	$\langle Reply,R, msgNum_i, Val,TS \rangle$ is in $M_i$
	\State \hspace*{0.2cm} $v \leftarrow$ Val corresponding to $t$
	
	\State \hspace*{0.2cm} \textbf{if} $t>r.ts_v$ \textbf{then}
    $r.value \leftarrow v$, $r.ts_v \leftarrow t$
	
	\State \textbf{else} \Comment{writeRequest}
	\State \hspace*{0.2cm} send $\langle writeRequest,msgNum_i,
	value,ts \rangle$  to all the processes in $cng.mem$
	\State \hspace*{0.2cm} \textbf{wait} until $\langle Reply,W,
	msgNum_i, OK \rangle$ is in $M_i$ from a majority of
	$cng.mem$  
	
	
	\State send $\langle readConf,msgNum_i \rangle$  to all
	processes in $cng.mem$   
	\State \textbf{wait} until $\langle Reply,C, msgNum_i,
	\ldots \rangle$ is in $M_i$ from a majority of $cng.mem$
	\State \textbf{for each} $\langle Reply,C, msgNum_i,
	Current \rangle \in M_i$
	\State \hspace*{1cm} \emph{updateCurrent(Current)}
 \EndProcedure\\

\Procedure{$RecursiveContact$}{$Request,cng,value,ts$}
	\State $ContactConfiguration(Request,cng,value,ts)$
	\State \textbf{if} $cng.ts < r.current.ts$
	\State \textbf{then} return 
	$RecursiveContact(Request,r.current,value,ts)$ 
	\State \textbf{elseif} $r.pending \neq \perp$ and $cng.ts <
	r.pending.ts$ 
	\State \textbf{then} return 
	$RecursiveContact(Request,r.pending,value,ts)$ 
	\State \textbf{if} $Request = readRequest$ \textbf{then} return
	$\langle r.value, r.ts_v \rangle$
	\State \textbf{else} return 
	\EndProcedure\\

\Procedure{$Read$}{}
	\State $opNum_i \leftarrow opNum_i + 1$
	\State $Op=\langle read  \rangle$
	\State $\langle v,ts \rangle \leftarrow
	RecursiveContact(readRequest, r.current, \perp, \perp )$ 
	\State  $RecursiveContact(writeRequest,r.current,v,ts)$ 
	\State  $Op= \perp$ 
	\State return v 
\EndProcedure\\

\Procedure{$Write$}{value}
	\State $opNum_i \leftarrow opNum_i + 1$
	\State $Op=\langle read  \rangle$
	\State $\langle v,ts \rangle \leftarrow
	RecursiveContact(readRequest, r.current, \perp, \perp )$ 
	\State$ts \leftarrow ts+1$ \State $Op=\langle  write, \ value,
	ts \rangle$ 
	\State  $RecursiveContact(writeRequest,r.current,v,ts)$ 
	\State  $Op= \perp$
	\State return ok 
\EndProcedure

\end{algorithmic}
\end{algorithm}


Before we present the $reconfig$ operation we have to describe
the $TwoPhaseUpdate$ procedure, which gets a set of changes
$Cng$, and makes from it a stable configuration.
First in lines 2-7 it combine $r.current$ with $Cng$ to a new
configration $Pending$. Next is sends $Pending$ (with indication
that it is pending configuration) to all the processes in
$r.current.mem$. Then, after receiving replay from a majority,
it reads the value that is stored in $r.current$ and write it to
$pending$ via $ReadFromConfiguration$ and
$WriteToConfiguration$. At this point $Pending$ is not pending
$configuration$ any more, and it is guaranteed that later
operation will not miss it. Then it sends again $Pending$ to all
the processes in $r.current.mem$, but this time as a stable
configuration. After receiving replays from a majority it sends
enable messages to all the new added processes. Process that
receives enable can start invoking operation.

A process $p$ that performs a $reconfig$ operation (line 19),
first sets $Op$ to be $reconfig$ and writes to it the set of
changes it wishes to make. Then in line 4 it sends 'what are you
doing' request to all the processes in $r.current.mem$, and
waits for their replay. When $p$ receives write replay it
updates its value. It also maintains three sets: $readset$ and
$writeset$ are contains processes that answers with $read$ and
$write$ correspondingly, and $Cng$ is a set of tuples s.t. every
tuple contains a process ID belonging to a process that answer
$reconfig$ and a set of changes is wish to make.

Now recall that $p$ cannot wait for replay from all the
processes because some of them could be faulty.
This is why we use $\diamond P_d$ oracle. For every process in
$r.current.mem$, $p$ waits either for a replay or for a
notification from the failure detector (FD) that the process
failed.

Next, in order to help the processes that perform $read$ and
$write$ operations, $p$ reads via
$recursiveRead$ and writes the returned value $val$ back via $recursiveWrite$. Notice that
$val$ is at least as updated as the most updated value among the
values that $p$ receives from the processes that
answer write. 
Then $p$ sends $val$ to all the processes in $readset$ and 'OK'
to all the processes in $writeset$. Process that receives such
a message can return from its operation (if it still performs
it). Before $p$ continues, it waits for acknowledgment from all
the processes (or notification from the FD). Otherwise it may be
the case that $p$ crashes immediately after completing
$reconfig$, and the messages will never delivered. 

Next $p$ helps, one be one, to the processes that performs
$reconfig$. For every tuple $\langle p_i,c \rangle \in Cng$, $p$
changes the $new$ configuration according to the changes in c,
and sends notification to $p_i$ (lines 30-35). Again for the
same reason as in $write$ and $read$, $p$ must wait for
acknowledgment from $p_i$ before continuing. 
 
In line 31, via procedure $consensus$ that we describe
before, $p$ tries to win the consensus object associated with
the $new$ configuration. But first recall that $p$ have to make
sure that the previous reconfig operation completed and $new$ is
no more pending configuration before proposing $c$.
Therefore, in line 31, $p$ calls to the consensus procedure with
$r.current$ (it is guaranteed that $r.current$ is not pending).

Now Notice that if many processes help the some process to add
some othe process $p_j$ then it may be the case that $p_j$ will
be added more than one time, and even worse, it may be added
then removed and then added again. In order to prevent this, we
assume that the consensus procedure returns $\perp$ if $c$ has
been already chosen before.

In line 33 it calls $TwoPhaseUpdate$ to make a configuration
from the set of changes returned from the $consensus$ procedure,
and to make it stable.

Now notice that if the condition in line 34 is satisfied, then
$c$ were not chosen, and instead of making new configuration
according the changes in $c$, $p$ helped completing
some previous $reconfig$ operation. In this case $p$ returns to
line 31 and tries again (this time $r.current$ is newer).

Each iteration completes when the condition in line 34 is not
satisfied, i.e. when $p$ receives from the consensus procedure
its own changes.
But it can happen only if $r.current$ is the $new$
configuration. It is easy to see that if $p$ runs alone, then
eventually $r.current$ will be the $new$ configuration. However,
with infinitely many concurrent $reconfig$ operation, it may
never happen. In this case some other process will eventually
help. 

After $p$ finishes helping other processes, it changes the $new$
configuration (in the same way) with its own changes (lines
36-39).
Then it set $Op$ to $\perp$ and returns. 

%%is it posibile that $p$ never receive such message?
%talk with idit about it! 
%what if $p$ always in the maniority?


%we make the consensus procedure return also a set of process
% that wes helped by this operation (with all the process from
% previous operation) ($p4 can propose it with Cng).
% Befor contiue $p$ will have to tale to all the prosess in that
% set. Process that answers is erased from the list and process
% that the failer detector says is failed stays in this list.

%the set can be big as the number of processes, newer operation
% of the same set erase the previous.


\begin{comment}
% old algorithm!
\begin{algorithm}[H]
% \floatname{algorithm}{ALGORITHM:}  
% \renewcommand{\thealgorithm}{}  
 \caption{Reconfiguration}  
 \label{alg:reconfiguration}
\begin{algorithmic}[1]

\Procedure{$TwoPhaseUpdate$}{$Cng$}
\State $Pending.mem \leftarrow r.current.mem$
\State \textbf{for all} $\langle add,p \rangle \in
	Cng$ \\ \hspace*{1cm} add $p$ to $Pending.mem$
\State \textbf{for all} $\langle remove,p \rangle
	\in Cng$ \\ \hspace*{1cm} remove $p$ from $Pending.mem$	
\State  $Pending.ts \leftarrow ts$,
	$Pending.pointer \leftarrow pointer$
\State  \textbf{to all} $p_i \in r.current.mem$ send $\langle
PC,Pending \rangle$ 
\State wait for majority to replay
\State $updatePending(Pending)$
\State ReadFromConfiguration($r.current$) 
\State WriteToConfiguration($Pending, r.value, r.ts_v$)
\State  \textbf{to all} $p_i \in r.current.mem$ send $\langle
NC,Pending \rangle$ 
\State wait for majority to replay
\State $updateCurrent(Pending)$
\State send $\langle enable, r.current \rangle$ to every process
$p$ s.t.
$\langle add,p \rangle \in Cng$ (or in pending?)
\EndProcedure\\

\Procedure{$reconfig$}{$cng$} \hspace*{1cm} 
$\backslash\backslash$ cng is a set of changes
\State $Op=\langle reconfig,  \langle
cng, \perp \rangle \rangle$ 
\State $writeset=\{\}, readset=\{\}, Cng=\{\}$ 
\State \textbf{to all} $p \in r.current.mem$ send $\langle
WhatAreYouDoing?\rangle$ 
\State  \textbf{for all} $p_i \in
r.current.mem$ wait for a replay or a notification from the
failure detector that $p_i$ failed.
	
	\State $\langle v,ts \rangle \leftarrow
	RecursiveRead(r.current)$
	% confuration and value from the processes in configure and
	% write it back to this configuration.
	
	\State RecursiveWrite($r.current, v, ts$)
	\State send $\langle opResponde, read,\langle v, ts
	\rangle \rangle$ to all the processes in $readset$
	\State  \textbf{for all} $p_i \in
	readset$ wait for an Ack or a notification from the
	FD that $p_i$ failed.
	% finish the operation only after complited the write to the
	% most update configuration! see figure in one of the papers on
	% the table. pay attention to New bit!
	\State send $\langle opResponde, write,ok \rangle$ to all the
	processes in $writeset$
	\State  \textbf{for all} $p_i \in
	writeset$ wait for an Ack or a notification from the
	FD that $p_i$ failed. 
	%\State  $configure$ $\leftarrow$ $r.current$
	
	\State \textbf{for all} $\langle p,c \rangle  \in Cng$
	\hspace*{1.2cm}$\backslash\backslash$ help one by one 
	 
	\State \hspace*{1cm}$\langle chosenCng,ts,pointer \rangle
	\leftarrow$ consensus($r.current$,$c$)
	\State \hspace*{1cm} \textbf{if} $chosenCng = \perp$
	\textbf{then} go to line 35 \hspace*{1cm}   
	$\backslash\backslash$ c was already added 
	 
	\State \hspace*{1cm} TwoPhaseUpdate($chosenCng$)
	\State \hspace*{1cm} \textbf{if} $chosenCng \neq c$
	\textbf{then} go to line 31  
	\hspace*{1.2cm}$\backslash\backslash$ c was not chosen
	
	\State \hspace*{1cm} send $\langle c, OK \rangle$ to $p$ and
	wait for Ack or a notification from the failure detector  that
	$p_i$ failed.
	
	\State $\langle chosenCng,ts,pointer \rangle
	\leftarrow$ consensus($r.current$,$cng$)
	\State \textbf{if} $chosenCng = \perp$
	\textbf{then} go to line 40
	 
	\State  TwoPhaseUpdate($chosenCng$)
	\State  \textbf{if} $chosenCng \neq c$
	\textbf{then} go to line 36  
	
	 %need to pay attention
	%to details- process may fail in the middle of the update!

	\State $Op= \langle \perp, \langle \perp, \perp \rangle
	\rangle$
	
\EndProcedure

\end{algorithmic}
\end{algorithm}
\end{comment}




\begin{algorithm}[H]
% \floatname{algorithm}{ALGORITHM:}  
% \renewcommand{\thealgorithm}{}  
 \caption{Reconfiguration}  
 \label{alg:reconfiguration}
\begin{algorithmic}[1]

\Procedure{$isReflected$}{$c,cng$}
	\State \textbf{if} $\forall \langle add,p \rangle \in c, p \in
	cng.mem \cup cng.removal$ \\ \hspace*{1cm} and $\forall \langle
	remove,p \rangle \in c, p \in cng.removal$ \textbf{then} return
	true
	\State \textbf{else} return false
\EndProcedure


\Procedure{$reconfig$}{$cng$}
\Comment{cng is a set of changes}
\begin{comment}
\State $Op=\langle reconfig,  \langle
cng, \perp \rangle \rangle$ 
\end{comment}
\State $opNum_i \leftarrow opNum_i + 1$
\State $Op= \langle reconfig, cng \rangle$


\State $ReadWriteSet=\{\}, Cng=\{\langle p_i,cng,opNum_i
\rangle \}$ 

\State \textbf{to all} $p \in r.current.mem$ send $\langle
WhatAreYouDoing?\rangle$ 
\State  \textbf{for all} $p_i \in
r.current.mem$ wait for a replay or a notification from the
failure detector that $p_i$ failed.
	
	\State $\langle v,ts \rangle \leftarrow
	RecursiveContact(readRequest, r.current, \perp, \perp )$
	% confuration and value from the processes in configure and
	% write it back to this configuration.
	
	\State $RecursiveContact(writeRequest, r.current, v, ts )$
	
	\begin{comment}
	\State send $\langle opResponde, read,\langle v, ts
	\rangle \rangle$ to all the processes in $readset$
	\State  \textbf{for all} $p_i \in
	readset$ wait for an Ack or a notification from the
	FD that $p_i$ failed.
	% finish the operation only after complited the write to the
	% most update configuration! see figure in one of the papers on
	% the table. pay attention to New bit!
	\State send $\langle opResponde, write,ok \rangle$ to all the
	processes in $writeset$
	\State  \textbf{for all} $p_i \in
	writeset$ wait for an Ack or a notification from the
	FD that $p_i$ failed. 
	%\State  $configure$ $\leftarrow$ $r.current$
	\end{comment}

	
	\State \textbf{for all} $\langle p,num \rangle \in
	ReadWriteSet$ send $\langle opHelp,num,v, ts \rangle$ to $p$
	
	
	\State \textbf{for all} $\langle p,num \rangle \in
	ReadWriteSet$ wait for $\langle Ack,num,p \rangle$ or a
	notification from the FD that $p_i$ failed.
	
	\State \textbf{for all} $\langle p,c,num \rangle  \in Cng$
	\Comment{help one by one, $\langle
	p_i,cng,opNum_i \rangle$ at the end} 
	
	\State \hspace*{1cm} \textbf{while}(!$isReflected(c,
	r.current)$) \State \hspace*{1.5cm} \textbf{while}(!\emph{test$\&$set(Pend)})
	\State \hspace*{1.5cm} \textbf{if}($isReflected(c,
	r.current)$) \textbf{then}
	\State \hspace*{2cm} $Pend \leftarrow false$
	\State \hspace*{2cm} \textbf{break}

	\State \hspace*{1.5cm} $r.current.propose(c)$
	
	\State \hspace*{1cm} send $\langle opHelp, num \rangle$ to $p$ 
	\State \hspace*{1cm} wait for $\langle Ack,num,p \rangle$ or a
	notification from the FD that $p$ failed. 
	
	

	 %need to pay attention
	%to details- process may fail in the middle of the update!

	\begin{comment}
	\State $Op= \langle \perp, \langle \perp, \perp \rangle
	\rangle$
	\end{comment}
	\State $Op=\perp$
	
\EndProcedure

  \Receiving{$\langle propose, current,c \rangle$ 
  from $p_i$} 
  \State \textbf{if} $current.ts < r.current.ts$ \textbf{then}
  return
  \State \textbf{else if} $current.ts > r.current.ts$
  \textbf{then}
  \State \hspace*{1cm} $Pend \leftarrow false$
  \State \hspace*{1cm} $r.current \leftarrow current$
  \State \hspace*{1cm} $r.pending \leftarrow \perp$
  \State \textbf{if} !\emph{test$\&$set(pend)} \textbf{then}
  $r.current.propose(c)$
  
  %naybe race!
  \EndReceiving
  
  \Upon{$r.current.decide(c)$}
  
  \State $r.pending.mem = \{p | (p \in r.current.mem \&\&
  \langle remove,p \rangle \notin c) || (\langle add,p \rangle
  \in c \&\& p \notin r.current.removal) \}$
  
  \State $r.pending.removal = \{p | (p \in r.current.removal ||
  \langle remove,p \rangle \in c \}$
  
  \State $r.pending.ts \leftarrow r.current.ts + 1$
  
  \State send $\langle r.pending,OK \rangle$  \textbf{to all}
  $p_j \in r.current.mem$
  \EndUpon


  
    \Receiving{$\langle r.pending,OK \rangle$ 
  		from majority of r.current.mem}

	\State $ContactConfiguration(readRequest, r.current, \perp,
	\perp )$
	\State $ContactConfiguration(writeRequest, r.pending, r.value,
	r.ts )$ 
	\State $r.current \leftarrow r.pending$
	\State $r.pending \leftarrow \perp$
	\State $pend \leftarrow false$ 

  \EndReceiving

\end{algorithmic}
\end{algorithm}

Algorithms~\ref{alg:messages} describe the
behavior of each process upon receiving messages.  








\begin{algorithm}[H]  
%\floatname{algorithm}{ALGORITHM:}  
%\enewcommand{\thealgorithm}{}  
\caption{}  
\label{alg:messages}

\begin{algorithmic}[1]


  \Receiving{$\langle WhatAreYouDoing? \rangle$ from $p_j$} 
     \State send $\langle operation,opNum_i, Op_i \rangle$ to
     $p_j$
  \EndReceiving
 
   \Receiving{$\langle operation, num, \langle read \rangle
   \rangle$ from $p_j$} 
   \State add $\langle p_j,num \rangle $ to $ReadWriteSet$
  \EndReceiving 
  
  \Receiving{$\langle operation, num, \langle write, value, ts
   \rangle \rangle$ from $p_j$} 
   \State add $\langle p_j,num \rangle $ to $ReadWriteSet$
  \State \textbf{if} $ts>r.ts_v$ \textbf{then}
  $r.value \leftarrow value, r.ts_v \leftarrow ts$
  \EndReceiving
  
   \Receiving{$\langle operation, num, \langle reconfig, cng
   \rangle \rangle$  from $p_j$} 
   \State $Cng \leftarrow Cng \cup \langle p_j, cng, num \rangle$
  \EndReceiving
   
   \Receiving{$\langle opHelp, num,v, ts \rangle$  from
   $p_j$}
   
   \State \textbf{if} $num \neq opNum_i$ \textbf{then} ignore
   \State \textbf{if} $Op = \langle write,\ldots \rangle$ or
   $\langle reconfig,\ldots \rangle$ \textbf{then} return OK
   \State \textbf{if} $Op =  \langle read \rangle$ \textbf{then} 
   $r.value=v$, $r.ts_v=ts$, and return $v$
   \State send $\langle Ack,num,p_i \rangle$ to $p_j$

  \EndReceiving   
  

\begin{comment}
   \Receiving{ $\langle PC,pending \rangle$   from $p_i$}
	 \State $updatePending(pending)$
     \State send $\langle PcReply,OK \rangle$ to $p_i$
  \EndReceiving   
  
   \Receiving{$\langle NC,current \rangle$  from $p_i$}
     \State $updateCurrent(current)$
      
     \State send $\langle NcReply,OK \rangle$ to $p_i$ 
     \State If the process is in the middle of an execution of 
      $reconfig(cng)$ s.t. \textbf{for all} $\langle add,p
      \rangle \in cng$, $p \in current.mem$ and \textbf{for all} 
      $\langle remove,p \rangle \in cng$, $p \notin current.mem$
      then it completes its $reconfig$ operation.
  \EndReceiving 

\end{comment}


 \Receiving{$\langle readConf,msgNum \rangle$  from $p_j$} 
     \State send $\langle Reply,C,msgNum, r.current  \rangle$ to
     $p_j$
  \EndReceiving

 \Receiving{$\langle readRequest,msgNum,\ldots \rangle$  from
 $p_j$} \State send $\langle Reply,R,msgNum, r.value, r.ts 
 \rangle$ to $p_j$
  \EndReceiving

   \Receiving{$\langle writeRequest,msgNum, value,ts \rangle$ 
   from $p_j$} 
   \State \textbf{if} $ts>r.ts_v$ \textbf{then}
   $r.value \leftarrow value$, $r.ts_v \leftarrow ts$ 
   \State send $\langle Reply,W,msgNum, OK  \rangle$ to $p_j$
  \EndReceiving
  
   \Receiving{$\langle Reply,\ldots \rangle$  from $p_j$} 
     \State add the message to $M_i$
  \EndReceiving 

\begin{comment}  
   \Receiving{$\langle readReply,R \rangle$  from $p_i$} 
     \State \textbf{if} $R.ts>r.ts_v$ \textbf{then}
     $r.Value \leftarrow R.value$, $r.ts_v \leftarrow R.ts$
  \EndReceiving   
   
 
  \Receiving{$\langle StatusReply,R \rangle$  from $p_i$} 
     \State $updateCurrent(R.current)$
     %\State $updatePeding(R.peding)$
  \EndReceiving 
\end{comment}
     
 
\end{algorithmic}
\end{algorithm}



\subsection{Correctness proof}
\label{sub:oracleProof}

TBD

\begin{comment}





We say that process is $enabled$ if it either part of the
initial configuration or receives $enable$ message.
We assume that only $enabled$ processes invokes operations.
\end{comment}

\subsubsection{Atomicity}


\begin{observation}

Only members of a $stable$ configuration can invoke operation. 

\end{observation}

\begin{proof}

The initial configuration is $stable$, and enable message 
is sent to new added process (line 16 in TwoPhaseUpdate) only
after the configuration, in which they were added, become
$stable$ (line 12 in TwoPhaseUpdate).

\end{proof}



\begin{observation}
\label{obs:order}

In every run $r$, the order of the configuration according to
their TS is corresponding to the order in which they were
generated. And in every time $t$ in $r$ there is exactly one
configuration, which associated consensus object has not been
won yet.

\end{observation}

\begin{proof}

Follow from the $consensus$ procedure.
Every configuration associated to a different consensus object.
Initially there is only the initial configuration, which
consensus object has not been won yet. New configuration can be
generated only by winning some consensus object, and consensus
objects may have at most one winner. The procedure associate new
TS to every generated configuration. 

\end{proof}

\begin{invariant}
\label{invariant}

At every time $t$ in a run $r$ of the algorithm, there is at
most one $pending$ configuration, and for every enabled process
$p_i$, $r_i.current$ holds a $stable$ configurations. 

\end{invariant} 

\begin{proof}

We prove by induction on the run.
Initially, at time 0, there is only the initial configuration
$c_0$.
This configuration is $stable$ by definition, and for every
$enabled$ process $p_i$,  $r_i.current=c_0$.

Now assume that the invariant holds for time $t=k-1$, we will
show that it is also holds for $t=k$.
There are three possible events at time $t=k$ that can possibly
violate the invariant: new added process receives $enable$
message, $enabled$ process updates its $r.current$ field, and
new pending configuration is generated.

Consider new added process $p_l$ receives $enable$ message
$m=\langle enable,conf \rangle$ at time $t=k$. Then $m$ must
have been sent at some time $t=k'<k$ by some other $enabled$
process $p_i$ (line 16 in $TwoPhasaUpdate$). By the assumption
$r_i.current$ hold $stable$ configuration at time $t=k'$.
Therefore $conf$ is stable configuration, and $r_l.current$ is
$stable$ configuration at time $t=k$.

Now consider some $enabled$ process $p_j$ updates its
$r_j.current$ field at time $t=k$. There is two places where it
can happens: Procedure $updateCurrent$ or $updatePending$.
Procedure $updateCurrent(cng)$ is invoked either in
$TwoPhaseUpdate(cng)$, after $cng$ becomes $stable$ or when
$p_j$ receives a message with current configuration from some
other enabled process. This message was sent before time $t=k$,
thus, by the assumption the configuration is $stable$.
In procedure $updatePending(cng)$, $r_j.current$ is updated only
if the TS associated with $cng$ is grater then the TS associated
with $r_j.pending$. By observation \ref{obs:order}, $cng$ was
generated after $r_j.pending$, and by the assumption there was only one
pending configuration at any time before time $t=k$. Therefore
at time $t=k$, $r_j.pending$ is no longer $pending$ and can be
written to $r_j.current$.

Now consider that new pending configuration is generated at time
$t=k$. It means that some $enabled$ process $p_n$ invoked
$consensus(r_n.current,chenges)$ procedure at some time
$t=k'<k$, and wins the consensus associated with $r_n.current$.
By the assumption $r_n.current$ is $stable$. By observation
\ref{obs:order}, the consensus objects associated with all the
configuration that were generated before time $t=k'$ have been
already won by time $t=k$. Now notice that procedure $consensus$
is called only with $r.current$ (line 31 in $reconfig$), and
again by the assumption $r.current$ is $stable$ configuration
for every $enabled$ process before time $t=k$. Therefore, at time
$t=k'$ there were no pending configuration, and in time $t=k$
there is at most one.

Hence, the invariant is holds for $t=k$.


\end{proof}


\begin{corollary}
\label{cor:order}

From the invariant follows that new
configuration is generated only after all the configuration,that
were generated before, become $stable$. Therefore the order of
the configuration according to their TS is corresponding to the
order according to the time in which they become $stable$. In
other words, if the TS associated with configuration $c$ is
bigger than the TS associated with configuration $c'$, then $c$
become $stable$ after $c'$.
%importent for the next Lemmas!

\end{corollary}


\begin{definition}

We say that a $write$ operation associated with TS $ts$ becomes
$stable$ when $RecursiveWrite$ procedure associated with TS
$ts' \geq ts$ completes.

\end{definition}

\begin{lemma}
\label{lem:help}

If during the execution of the recursive procedures
$RecursiveWrite$ and $RecursiveRead$ there is a recursive call
with a $pending$ configuration at time $t$, then there was a
recursive call with the previous configuration before, and this
configuration is $stable$ at time $t$.

\end{lemma}

\begin{proof}

Consider a recursive call of $RecursiveWrite$ or $RecursiveRead$
procedure with a $pending$ configuration $c_c$ at time $t$.
Notice that this recursive call is not the first, because the
procedure is called with $r.current$, and by Invariant
\ref{invariant}, $r.current$ holds a $stable$ configuration.
Now consider the previous call $rec$, which was called with the
configuration $c_p$. By the run of the algorithm $c_c$ was
observed, and no configuration older than $c_c$ and newer than
$c_p$ was observed during $rec$. Now assume by the way of
contradiction that $c_p$ is not the previous configuration of
$c_c$. Hence, by Invariant \ref{invariant}, there is a $stable$
configuration that was not observed by $rec$. Now notice, in
Algorithm \ref{alg:update}, that processes do not forget
$stable$ configuration until newer $stable$ configuration is
observed. Therefore, during the execution of $rec$, a $stable$
configuration newer than $c_p$ and older than $c_c$ must have
been observed, and thus the next recursive call after $rec$ must
have been called with $stable$ configuration, denote it $c_s$.
Contradiction. By invariant \ref{invariant}, $c_s$ is $stable$ at
time $t$.

\end{proof}

\begin{lemma}
\label{lem:write1}

Assume some $write$ operation, associated
with TS $ts$, becomes $stable$ at time $t$ in a run $r$. Then
there is a time $t'<t$ s.t. there is a majority of the newest
$stable$ configuration at time $t$ that holds a $value$ that is
associated with some TS $ts'$ s.t. $ts' \geq ts$. 

\end{lemma}

\begin{proof}

Consider the $RecursiveWrite$ procedure that makes the $write$
$stable$ at time $t$, denote it $rw$. By definition $rw$
completes at time $t$. Now consider its last recursive call
$rec$, and assume that $rec$ was called with configuration $c$.
Denote the $WriteToConfiguration$ called by $rec$ to be $wtc$.
Procedure $wtc$ write to a majority of $c$ and read the
configuration status from a mojority of $c$. The $rw$ returned,
so $wtc$ didn't found any configuration newer than $c$ in a
majority of $c$. Now recall that a configuration becomes
$stable$ only after a majority of the previous configuration
receives it. Therefore there is a time $t'<t$ after the majority
of $c$ receives $\langle value,ts\rangle$, in which there is no
$stable$ configuration newer than $c$. If $c$ is a $stable$
configuration, then we done. If not, then by Lemma
\ref{lem:help} there was a recursive call of $rw$ with the
previous configuration, and
therefore a majority of this configuration received the write
before time $t'$, denote this configuration to be $c'$. Again by
Lemma \ref{lem:help} $c'$ is $stable$ at time
$t'$, thus $c'$ is the newest $stable$ configuration at
time $t'$. Notice that processes overwrite their values only
with bigger TS. The Lemma follows.




\end{proof}

\begin{lemma}
\label{lem:write2}

Assume some $write$ operation, associated with TS $ts$, 
becomes $stable$ at time $t$ in a run $r$. Then there is a time
$t'<t$ s.t. for any configuration $c$ that becomes $stable$
after $t'$, there is a majority of $c.mem$ that holds a $value$
that is associated with some TS $ts'$ s.t. $ts' \geq ts$.

\end{lemma}

\begin{proof}

By Lemma \ref{lem:write1}, there is a time $t'$ s.t. there is a
majority of the newest $stable$ configuration at time $t'$ that
holds a $value$ that is associated with some TS $ts'$ s.t. $ts'
\geq ts$. Now recall that processes never update
their $value$ with smaller TS. Recall also that $pending$
configuration becomes $stable$ only after a $value$ that is read
from a majority of the previous configuration is written to a
its majority. The Lemma follows by simple induction.  



\end{proof}


\begin{lemma}

Assume some $RecursiveRead$ procedure $rec$, that invokes at
time $t$, completes at time $t'$, and returns
$\langle value, ts \rangle$. Then there is a time $t<t''<t'$
s.t. there is a majority of the newest $stable$ 
configuration at time $t'$ s.t. every process in this majority
holds a $value$ associated with a TS not greater the $ts$ at
time $t''$.


\end{lemma}

\begin{proof}

Denote $rec$'s last recursive call to be $last$, and assume that
$last$ was called with configuration $c$. $last$ read the value
from a majority of $c$, and then read the status of the
configurations from a majority of $c$ via
$readFromConfiguration$. Denote the time at which $last$
started to read to be $t_c$. Now notice that procedure $rec$
returns, so no configuration newer than $c$ was observed during
$last$. Therefore at time $t_c$ there is no 
$stable$ configuration newer than $c$. If $c$ is $stable$, then
$t''=t_c$ and we done. Else, by Lemma \ref{lem:help}, there was
a recursive call of $rec$ with the previous $stable$
configuration of $c$. Denote this recursive call to be $prev$
and the configuration to be $c'$. Now denote the time at which
$prev$ called $readFromConfiguration$ to be $t_p$. At time..

Consider the last $readFromConfiguration(c)$ procedure that were
invoked by $rec$. This procedure completes, thus there is a
majority of $c$ s.t. every
process in this majority holds a $value$ associated with a TS
that is not greater the $ts$.

\end{proof}

\begin{corollary}
????
Assume some $RecursiveRead$ procedure $rec$, that invokes at
time $t$, completes at time $t'$, and returns
$\langle value, ts \rangle$. Then there is a time $t<t''<t'$
s.t. there is a majority of the newest ($stable$ or $panding$)
configuration at time $t''$ s.t. every process in this majority
holds a $value$ associated with a TS not greater the $ts$. 


\end{corollary}

\begin{proof}



\end{proof}

Notice that every $read_i$ operation returns a $value$ that is
obtained by a $RecursiveRead$ procedure. This procedure is
either invoked by $p_i$ (line 30 in procedure $read$) or by some
other process $p_j$ during its $reconfig$ operation (line 25 in
procedure $reconfig$) when it helps $p_i$. We say that the TS
associated with the $value$ returned by $read_i$ is the TS
returned by the $RecursiveRead$ procedure that obtained the
$value$.

\begin{lemma}

If $write$ operation $w$ completes before $read$ operation $r$
invoked, then the TS associated to $w$ is less then or equal to
the TS associated with the value returned by $r$.

\end{lemma}

\begin{proof}

\end{proof}

\begin{lemma}

If $write$ operation $w$ completes before $write$ operation $w'$
invoked, then the TS associated to $w$ is less then
the TS associated to $w'$


\end{lemma}

\begin{proof}

\end{proof}

\begin{lemma}

If $read$ operation $r$ completes before $read$ operation $r'$
invoked, then the TS associated with the value returned by $r'$
is less then or equal to the TS associated with the value
returned by $r'$.

\end{lemma}

\begin{proof}

\end{proof}


\begin{lemma}

If $read$ operation $r$ completes before $write$ operation $w$
invoked, then the TS associated to $w$
is greater than the TS associated with the value
returned by $r$.


\end{lemma}

\begin{proof}

\end{proof}

\begin{theorem}

The algorithm implements an $dynamic$ $atomic$ storage in $D_3$

\end{theorem}

\begin{proof}

Similarly to ABD and Dynastore.

\end{proof}



\begin{comment}
\begin{definition}

Notice that every $read_i$ operation returns a $value$ that is
obtained by a $RecursiveRead$ procedure. This procedure is either
invokes by $p_i$ (line 30) or by some other process $p_j$ during
its $reconfig$ operation (when it helps $p_i$). We say that a
$read$ operation becomes $stable$, when the $RecursiveRead$ that
obtain its $value$ completes.

\end{definition}
\end{comment}






\subsubsection{Liveness properties}

%Lemma:
%The liveness properties guarantee that a majority of the most
%stable configuration alive




==> sections/dynamicAtomicSnapshot.tex <==
\section{Dynamic Atomic Snapshot in $D_3$}
\label{sec:snap}

In the previous section we showed that mutable objects, and in
particular snapshots, cannot be simulated from SWMR
registers in $M_2$. In this section we show that model $D_2$ is
stronger than $M_2$, and model $D_3$ is stronger than $M_3$,
presenting an algorithm that simulates a dynamic snapshot
object in model $D_3$ from SWMR registers only. The algorithm is
given in Section 5.1, and its correctness is proven in Section
5.2.
then. We show how to use snapshot in order to simulate a dynamic
MWMR register in $D_3$ (Section 5.3).
This, in turn, allows every dynamic object that can be simulated
from MWMR registers in $M_3$, For example, a dynamic counter
\cite{aguilera2004column}, to be simulated in $D_3$ using SWMR
registers.



 
\subsection{Algorithm}

The general idea of the algorithm is based on the well known
snapshot algorithm for static systems \cite{snaoshot}. Each
process writes to a \emph{segment}, which is a SWMR register
that holds its data (written by its last \textit{update}) and
some additional information.
A process that performs a $scan$ operation repeatedly collects
all the segments until it gets two identical scans, which is
called a successful \emph{double collect}. The mapping of process
to data read from their segment in this collect, also called
$view$, is stored in the segment.
Notice that if other processes perform infinity many updates concurrently with the $scan$, it may never obtain a double collect.
In order to overcome this, the algorithm uses a helping
mechanism, whereby a process that fails to obtain a successful
double collect a certain number of times, (at most $2n+1$ in the
original algorithm), can borrow a view from another process.


Now recall that in $D_3$, two additional atomic operations have
to be supported, $add$ and $remove$, which change the set of
processes that can invoke operations and the set of values
that should be returned by a $scan$ operation. In order to deal
with configuration changes, we extend the
view embedded in the segment to hold two fields.
The first, denoted $mem$, is the set of all known added
processes. Note that in the original algorithm, this set is
constant, thus there is no need to store it in the segment.
The second field is an array of size $|mem|$, (instead of a
constent $n$ in the original algorithm), denoted by $snap$,
where $snap[i]$ hold the last data value read from $segment_i$.
Initially, $mem$ is the set $P_0$.

But still some problems arise. The first problem is how
a process that performs a $scan$ operation can determine which
processes are in the $current$ set. In order to solve this, we
add to every segment an array of reconfigurations, denoted
$changes$. A process that performs $add$ or $remove$ writes the
operation to $changes$. A process that begins a $scan$, first
collects the segments that belong to the processes in its $mem$,
then checks their $changes$ arrays to discover which processes
were added or removed, and then updates its view ($mem$ and
$snap$) accordingly.
Notice that the shared memory is reliable and segments of
removed processes remain in memory.
Therefore, information about added and removed processes is never
lost, and even slow processes can obtain it.
 
The second problem that arises in $D_3$ is how a
process can know which view can be borrowed during a $scan$
operation. Consider a run, illustrated in Figure
\ref{fig:changes}, in which some process performs a $scan$
concurrently with infinitely many $add$ operations,
s.t. every new process performs exactly one $add$ and no
updates. One way for a scan to complete is by obtaining
a successful double collect, but in this case, because of the
infinitely many $add$ operations, the $scan$ can never obtain
one despite the fact that there are no updates. Alternatively,
the scan can borrow a view from another process, but it needs to
make sure that the view is fresh enough. To this end,
we add a version number, denoted $num$, to every segment. Each
process increases its $num$ at the beginning of every $scan$
operation, and in every collect it checks whether some process
has a view that contains its updated $num$. If some process has
such a view, then it means that this view is fresh and can be
borrowed.

The segment structure is defined in
Algorithm \ref{alg:segment} and illustrated in Figure
\ref{fig:segment}. The algorithm is presented in Algorithms 2--6.

In the context of our algorithm, we say that a \textit{process
$p_i$ has been added before time $t$} in a run $\sigma$ of the
algorithm if $p_i \in P_0$ or some other process $p_j$
wrote $\langle add,p_i \rangle$ to its segment during $add(p_i)$ operation (line 4 in
Algorithm \ref{alg:add}) before time $t$, in the same way we say,
that a \textit{process $p$ has been removed before time $t$} in
$\sigma$ if some other process wrote $\langle remove,p\ \rangle$
to its segment during $remove(p_i)$ (line 3 in Algorithm
\ref{alg:remove}) before time $t$. In the next section we show
that these embedded writes are
also the linearization points of the $add$ and $remove$
operations.

\begin{comment}
 The $update$ operations are linearized at the same time in the
 run as their embedded write (line 3 in Algorithm
 \ref{alg:update}) to their segments.
\end{comment}

In a given run $\sigma$, we define \textit{full snapshot(t)} to
be the state of the shared memory variables of processes added
before time $t$, at time $t$.
That as,\textit{full snapshot(t)} is a mapping from each
processes that has been added before time $t$ to the value
$\langle value,changes,num \rangle$ that was last written to
$segment_{i_j}$ before time $t$ in $\sigma$.




We define \textit{snapshot(t)} to be the sub-mapping of
full-snapshot(t) excluding processes removed before time $t$.


The core of the algorithm lays in the \textit{embaddedScan}
procedure, which returns a \textit{full snapshot(t)} for some
$t$ that is later than the time when the procedure began. 
Helping is achieved by performing the embaddedScan
at the beginning of every operation ($scan$, $update$, $add$,
and $remove$) and saving its result in the view field of the
segment.


 
\begin{figure}[ht]      
  \centering 
  \includegraphics[width=6in]{changes}
  \caption[segment]
   {Run with infinitely many changes.}
   \label{fig:changes}
\end{figure}



\begin{algorithm}[H]
 \caption{Segment structure}
 \label{alg:segment}
\begin{algorithmic}

 
%\State $\Pi = \{p_1,p_2,....\}$.

\State $\mathcal{L}=\langle\{add,remove\} \times \Pi \rangle^{\ast}$ 
\hspace{3cm}$\backslash\backslash$ arrays of changes
\State $segment = \langle val, changes , num, view \rangle $ 
\\ \hspace*{1cm}  where $val \in \mathcal{V}$, $changes \in
\mathcal{L}$, $num \in \mathbb{N}$, $view=\langle mem,
snap \rangle$
\\ \hspace*{2cm} where $mem \subset \Pi$, and $snap$ is an array
of size $|mem|$ \\ \hspace*{2cm} s.t. $snap[i]=\langle
val,changes,num \rangle$ 
\\ \hspace*{3cm} where $val \in \mathcal{V}$, $changes \in
\mathcal{L}$, $num \in \mathbb{N}$ 

\State $P_0\subseteq \Pi$
\State $View_0=\langle P_0, \langle \perp, [$ $], 0\rangle^{|P_0|}
\rangle \rangle$
\State $\forall p_i \in \Pi$, $segment_i$ readable by all,
writable by $p_i$ 
\\ \hspace*{1cm} \textbf{initially:} if $p_i \in P_0$,
$segment_i=\langle \perp, [$ $], 0, View_0 \rangle$
\\ \hspace*{2.9cm} else $segment_i=\perp$





\end{algorithmic}
\end{algorithm}


\begin{figure}[ht]      
  \centering 
  \includegraphics[width=6in]{segment}
  \caption[segment]
   {Example of $segment_1$. In this example $P_0=\{ p_1,p_2\}$,
   process $p_2$ does not invoke any operation yet, and process
   $p_1$ completes \emph{add($p_3$)}, including writing 1 to
   $segment_1.num$, performing \emph{embeddedScan} and writing
   the result to $segment_1.view$, and finally writing $\langle
   add,p_3 \rangle$ to $segment_1.changes$. }
   
   \label{fig:segment}
\end{figure}

We now describe the algorithm, which presented in details in
Algorithms 2--6. Operation $scan$ (Algorithm~\ref{alg:scan})
first performs $embeddedScan$ in line 2. Then in line 3 it checks
which of the processes were removed.
Finally in lines 4--6 it returns a map that maps every process
that was added but not removed to its segment value. The
$update$ operation (Algorithm~\ref{alg:updated}) first performs
$embeddedScan$ and then writes the new value to the segment.

 
\begin{algorithm}[H]
  \caption{}
  \label{alg:scan}
\begin{algorithmic}[1]



\Procedure{$scan_i()$}{}
	\State $embeddedScan()$
	\State $removedSet \leftarrow \{ p$ $|$ $\exists j$ s.t  $
	\langle remove, p \rangle \in segment_i.View.snap[j].changes \}$
	
	\State $\forall p_j \in segment_i.View.mem \setminus
	removedSet$ \\ \hspace{1cm} $V[j]=segment_i.View.snap[j].Value$ 
	\State return V
\EndProcedure

\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
  \caption{}
  \label{alg:updated}
\begin{algorithmic}[1]

\Procedure{$update_i$}{$d$}
	\State $embeddedScan()$
	\State $segment_i.value \leftarrow d$
\EndProcedure

\end{algorithmic}
\end{algorithm}

In order to perform an $add$
(Algorithm~\ref{alg:add}) or $remove$
(Algorithm~\ref{alg:remove}), processes first perform
$embeddedScan$ and then add to their changes list the
information about the removed or added process.
Additionally, in the $add$ operation, the initial
value of the new added segment is set. 

\begin{algorithm}[H]
  \caption{}
  \label{alg:add}
\begin{algorithmic}[1]

\Procedure{$add_i$}{$p_j$}
	\State $embeddedScan()$ 
	\State Set $segment_j$'s initial value to be $\langle 
	\perp,[$ $],0,segment_i.View \rangle$   
	\State Insert $\langle add, p_j \rangle$ to first empty cell in
	$segment_i.changes$ 
	
\EndProcedure


\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
  \caption{}
  \label{alg:remove}
\begin{algorithmic}[1]

\Procedure{$remove_i$}{$p_j$}
	\State $embeddedScan()$
	\State Insert $\langle remove, p_j \rangle$ to first empty cell
	in $segment_i.changes$ 
		
\EndProcedure

\end{algorithmic}
\end{algorithm}

We are ready now to present the $embeddedScan$ procedure
(Algorithm~\ref{alg:embeddedScan}), which is used by all
operations. A process $p_i$ that performs an $embeddedScan$
first increases its version number in shared memory (line
\ref{line:vn}), and then begins repeatedly collecting segments
of all known added processes (lines
\ref{line:collect1}--\ref{line:collect2}), which are stored in
$PrevView.mem$.

The procedure uses two local variables to trace the added
processes and their views, $CurView$ and $PrevView$. They both
store a view, which has two fields, $mem$ that stores the known
added processes, and $snap$ that stores the collect of all the
processes in $mem$. In every iteration after the first,
$PrevView$ stores the view from the previous iteration, and in
the first iteration the view from $p_i$'s segment.
$CurView$ stores the view obtained by the collect in the
current iteration.
In lines \ref{line:updateView1}--\ref{line:updateView2},
$PrevView$ is updated according to $CurView$, all the new added
processes that were observed in the $changes$ arrays in
$CurView.snap$ are added to $PrevView.mem$.

There are two ways for $p_i$ to complete the $embeddedScan$. The
first is by obtaining a successful double collect in line
\ref{line:dubblecollect}.
The second is by borrowing the view of another process that
contains $p_i$'s updated version number
(\ref{line:borrowBegin}--\ref{line:borrowEnd}). It is guaranteed
that this view was obtained after $p_i$'s $embeddedScan$ began
because version numbers never decrease, and this number is
increased at the beginning of the $embeddedScan$.

Finally, in line \ref{line:stop}, $p_i$ checks if it was removed, and
if so, then it stops. Otherwise $p_i$ writes the new view to
its segment in line \ref{line:writeToSeg}.


\begin{algorithm}[H]
  \caption{}
  \label{alg:embeddedScan}
\begin{algorithmic}[1]
\small 
\Procedure{$embeddedScan()_i$}{}

	\State $PrevView \leftarrow segment_i.view$
	\label{line:readFromSeg} 
	\State $segment_i.num \leftarrow segment_i.num+1$
 	\label{line:vn}  
	\Comment{Increase version number}
	\Statex
	
	\While{true} \Comment{Waiting for consistent
	snapshot}

		\State 	$CurView.mem=PrevView.mem$
		\label{line:collectBegin}
		
		\State \textbf{for each} $p_j \in CurView.mem$
		\label{line:collect1}
		\State \hspace{0.5cm} $CurView.snap[j]=\langle
		segment_j.value,segment_j.changes, segment_j.num \rangle$
		\label{line:collect2}
		\begin{comment}
		\State $\forall p_j \in CurView.mem$, $CurView.snap[j]=\langle
		value,changes, num \rangle $ \\ \hspace{2cm} where
		$value=segment_j.value$, $changes=segment_j.changes$, \\
		\hspace{2cm} $num=segment_j.num$
 		\end{comment}
 		
		\State \textbf{if} \textit{CurView=PrevView} \textbf{then} goto
		\textbf{Done}
		\label{line:dubblecollect} 
		\Comment{Successful double collect}
		
		\For{\textbf{each} $P_j \in CurView.mem$ s.t.
		$PrevView.snap[j] \neq CurView.snap[j]$}
			
			\If {$segment_j.View.Snap[i].num = segment_i.num$}
			\label{line:borrowBegin}
			\Comment{Found fresh snapshot} 
			\State $CurView \leftarrow segment_j.view$
			\State goto
			\textbf{Done}
  			\EndIf
  			\label{line:borrowEnd}
  		  
  			\Statex \Comment {Update
  			view}
  			
  			\State \textbf{for each} $\langle add, p_l \rangle \in
  			CurView.snap[j].changes \setminus PrevView.snap[j].changes$
  			\label{line:updateView1}
  				\State \hspace{3.5cm}$PrevView.mem \leftarrow
  				PrevView.mem \bigcup \{p_l\}$ 
				\State \hspace{3.5cm}$PrevView.snap[l] \leftarrow
					\langle \perp ,[$ $],0 \rangle$ 

			\State $PrevView.snap[j] \leftarrow CurView.snap[j]$
			\label{line:updateView2}
		\EndFor

	\EndWhile 
 	\Statex
	\textbf{Done:}
	
	\State \textbf{If} $\exists j$ s.t. 
	$\langle remove, p_i \rangle \in CurView.snap[j].changes$
	\textbf{then} stop
	\Comment{$p_i$ was removed}
	\label{line:stop}

	\State $segment_i.view \leftarrow CurView$
	\label{line:writeToSeg}
\EndProcedure


\end{algorithmic}
\end{algorithm}

\subsection{Correctness}


\begin{observation}
\label{obs:p0}

Consider some time t in a run $\sigma$ when some process $p_i$
is executing $embeddedScan$.
Then $P_0 \subseteq PrevView_i.mem$ at time t.

\end{observation}

\begin{proof}

Recall that, initially, $segment_k.view.mem = P_0$ for every 
process $p_k \in P_0$. Now notice that $segment_i.view$ is read
into $PrevView_i$ at the beginning of every $embeddedScan_i$
(line \ref{line:readFromSeg} in
Algorithm~\ref{alg:embeddedScan}), and is written back at the
end (line \ref{line:writeToSeg} in
Algorithm~\ref{alg:embeddedScan}).
Notice also that no process is taken out of $PrevView_i.mem$
during an $embeddedScan$, and that $embeddedScan_i$ is
the only procedure in the algorithm where $segment_i.view$ is
written.
Therefore, the observation holds for all processes in $P_0$.
Now notice that an added process inherits its view from the
process that adds it (line 3 in
Algorithm~\ref{alg:add}). Recall that only process in $current$
set can add new process. Thus, it is easy to show by
induction that the observation holds for every added process.

\end{proof}


\begin{lemma}
\label{lemma:list} 


 Consider some time t in a run $\sigma$ when some process $p_i$
 is at the beginning of some collect in an execution of
 $embeddedScan$ (line \ref{line:collectBegin} in Algorithm
 \ref{alg:embeddedScan}).
 Now assume that there is a process $p_j \notin
 PrevView_i.mem$ at time t, which has been 
 added before time t. Then there exists $p_k \in
 PrevView_i.mem$ s.t.
 $PrevView_i.Snap[k].changes \neq segment_k.changes$ at time t. 
 

 
\end{lemma}

\begin{proof}

Process $p_j$, denoted also $p_{j_0}$, has been added before
time $t$ by some process $p_{j_1}$. Process $p_{j_1}$ is either
in $P_0$ or it has been added by another process $p_{j_2}$
before time $t$. Process $p_{j_2}$ is also either in $P_0$ or it
has been added by another process $p_{j_3}$ before time $t$.
The number of added processes before time $t$ is finite. Thus,
there is a sequence $p_{j_0},p_{j_1},\ldots,p_{j_n}$ s.t. for
every $0 \leq l<n$ process $p_{j_l}$ has been added by
$p_{j_{l+1}}$, and $p_{j_n} \in P_0$. Now consider the process
$p_{j_k}$ with the lowest $k$ s.t. $p_{j_k} \in PrevView_i.mem$
at time $t$. It is guaranteed that there is such a process
because $p_{j_n} \in P_0$ and by Observation \ref{obs:p0}, $P_0
\subseteq PrevView_i.mem$ at time $t$.
Process $p_{j_{k-1}}$ has been added by $p_{j_k}$ before time
$t$, so $segment_{j_k}.changes$ contains $\langle add,
p_{j_{k-1}} \rangle$ (line 4 in Algorithm \ref{alg:add}) at time
$t$, whereas $PrevView_i.Snap[j].changes$ does not, otherwise
$p_i$ would have added $p_{j_{k-1}}$ to $PrevView_i.mem$ in the
an earlier (lines 16-19 in Algorithm
\ref{alg:embeddedScan}).
\end{proof}

\begin{corollary}
\label{cor:listInverse}

 Consider some time t in a run $\sigma$ when some process
 $p_i$ is at the beginning of some collect in an execution of
 $embeddedScan$ (line \ref{line:collectBegin} in Algorithm
 \ref{alg:embeddedScan}).
 If $PrevView_i.Snap[j].changes =segment_j.changes$ for all
 $p_j\in PrevView_i.mem$, then $PrevView_i.mem$ contains at time
 $t$ all the processes that have been added before time $t$.


\end{corollary}

\begin{lemma}
\label{lem:doublecollect}


Assume some process $p_i$ completes a successful double
collect in a run $\sigma$ during an execution of $embeddedScan$
(line \ref{line:dubblecollect} in Algorithm
\ref{alg:embeddedScan}). And assume that the second collect
begins at time $t$. Then at time $t$,
$PrevView_i.snap=\textit{full snapshot(t)}$, and the value
written to $segment_i.view$ at the end of the $embeddedScan$ is
\textit{full snapshot(t)}.

\end{lemma}

\begin{proof}

Recall that at time $t$, $PrevView_i.snap$ holds the value that
was returned from the first collect. 
We first show that $\forall p_k \in PrevView.mem$,
$PrevView.snap[k]$ is equal to $segment_k$ at time $t$. Assume
the contrary, then $p_k$ wrote to $segment_k$ in the interval
between the read of $segment_k$ in the first collect and time
$t$. The values of $segment_k$ cannot repeat themselves because
$segment_k.num$ is increased at the beginning of every
operation. Therefore, the value that was read from $segment_k$ in
the second collect is different from the value that was read
from $segment_k$ in the first collect.
A contradiction to the successful double collect.
We get that at time $t$, $PrevView_i.Snap[j] =
segment_j$, for each $p_j \in PrevView.mem$ and, in particular,
$PrevView_i.Snap[j].changes = segment_j.changes$ for all $p_j
\in PrevView.mem$. By Corollary \ref{cor:listInverse},
$PrevView.mem$ contains at time $t$ all the processes that have
been added before time $t$. And therefore, at time $t$,
$PrevView.snap$ is the $\textit{full-snapshot(t)}$. After a
successful double collect, $p_i$ stops the iterations and in
line \ref{line:writeToSeg} writes $PrevView_i$ to its segment.


\end{proof}

\begin{lemma}
\label{lem:borrowing}


Consider some process $p_i$ that begins an $embeddedScan$ at
some time $t$. If at some later time $t_1>t$ during the
execution of the $embeddedScan$, $p_i$ reads some 
$segment_j$ s.t.
$segment_j.view.snap[i].num = segment_i.num$ (the condition in
line \ref{line:borrowBegin} in Algorithm
\ref{alg:embeddedScan}), then the value of $segment_j.view.snap$
at every time after time $t_1$ is a \textit{full snapshot(t')}
for some $t'>t$.  %And therefore can be returned by $p_i$'s $embaddedScan$.

\end{lemma}

\begin{proof}

Let $V$ be the value of $segment_j.view$ at some time $t_2>t_1$.
This value was either obtained by a successful double collect or
borrowed from another process. Consider it was borrowed from
another process $p_k$. Process $p_k$ could have obtained the
value by a successful double collect or again by borrowing it from
anther process. This argument can be applied inductively. Note
that there is a finite number of processes that were added before
time $t_2$.
Hence, eventually this value must has been obtained by a
successful double collect.
Assume it was obtained by a successful double collect $D$ by
a process $p_l$. 
Now recall that process $p_i$ increases $segment_i.num$ at the
beginning of its $embaddedScan$.
From the condition in line \ref{line:borrowBegin} (Algorithm
\ref{alg:embeddedScan}) we get that $p_l$ reads $p_i$'s segment
during the first collect of $D$, after $p_i$ increases its
version number, i.e., after
time $t$.
Denote the time at the beginning of the second collect of D by
$t'$ (notice that $t'>t$). By Lemma
\ref{lem:doublecollect}, the value of $PrevView_l.snap$ at $t'$
is the \textit{full-snapshot(t')}. Therefore $V$ is the
\textit{full-snapshot(t')}.

It follows that the value of
$segment_j.view.snap$ at every time after time $t_1$ is a
\textit{full snapshot(t'')} for some $t''>t$.  




\end{proof}

\begin{corollary}
\label{cor:scan}

Consider a run $\sigma$ in which some process $p_i$ invokes a
$scan$ operation at time $t$. Now assume that the $scan$
operation completes at some time $t_1>t$ and returns $V$.
Then $V$ is a \textit{snapshot(t')} for some $t<t'<t_1$.

\end{corollary}


\begin{proof}

The $scan$ operation begins by performing $embaddedScan$,
which completes either by a successful double collect or by
borrowing the $view$, $S$, from another process. 
By Lemmas \ref{lem:doublecollect} and \ref{lem:borrowing}
respectively, the $embaddedScan$ returns a
\textit{full-snapshot(t')} for some $t<t'<t_1$. Now recall that,
be our definition, a process $p$ has been removed before time
$t'$ in run $\sigma$ if some other process $p_j$ wrote $\langle
remove, p \rangle$ to $segment_j.changes$.
Since $S$ is a \textit{full-snapshot(t')}, it holds all the
information about processes that have been removed before time
$t'$. Therefore, in lines 3--5 in Algorithm \ref{alg:scan},
$p_i$ discards all the processes that have been removed before
time $t'$, and returns \textit{snapshot(t')} in line 6.



\end{proof}

\begin{lemma}
\label{lem:wait-free}

The algorithm is wait-free in $D_3$.

\end{lemma}

\begin{proof}

In order to show that the algorithm is wait-free we only have to
show that $embeddedScan$ is wait-free. Now consider some run
$\sigma$ in which some process $p_i$ begins $embeddedScan$, and
increases $segment_i.num$ at time $t$. Notice that every
$embeddedScan$ that begins after time $t$ reads the updated
$segment_i.num$. Therefore, every operation by some process $p_j
\in PrevView_i.mem$ that begins after time $t$ and writes to
$segment_j$ causes the condition in line
\ref{line:borrowBegin} of $p_i$'s $embeddedScan$ to be satisfied, which lead
to the $embeddedScan$'s completion.

The number of processes that have been added before time $t$ is
finite, and only added processes can invoke operations, and each
process invokes at most one operation at a time. Thus, 
a finite number of operations begin before time $t$. 
Since every unsuccessful collect sees at least one new operation
that writes to some $segment_j$ during $embeddedScan$,
after a finite number of double collects $p_i$ 
either succeeds to double collect or borrows a view from another
process, and the $embeddedScan$ completes.   

\end{proof}

\begin{theorem}

The algorithm implements a wait-free atomic snapshot in $D_3$.



\end{theorem}

\begin{proof}

The algorithm is wait-free by Lemma \ref{lem:wait-free}. It is
left to show that the algorithm is atomic. The
linearization points for $add$, $remove$, and $update$ are the
times when they write to the process's segment (line 3 in
Algorithms \ref{alg:updated},\ref{alg:remove} and line 4 in
Algorithm \ref{alg:add}). Recall that a $scan$ operation returns a value $V$ that is \textit{snapshot(t')} for
some t' in the $scan$'s execution interval. We let $t'$ be
a linearization point for the $scan$. The atomicity of the
algorithm with these liveness points stems from Corollary
\ref{cor:scan}.

\end{proof}

\subsection{MWMR register in $D_3$}

We can use a dynamic snapshot object to implement an MWMR
register in $D_3$. The snapshot object's update operation is
used to the data written to the register and a time stamp.
In order to read the register's value, a process performs a
$scan$ and return the data associated with the biggest time
stamp.
Ties are broken by process ids. In order to write,
a processes first performs $scan$ and picks a larger times tamp
then all those obtained, and then calls $update$ with the new
data and time stamp. 
Operation $add$ is implemented by invoking the $add$ of the
snapshot object, and $remove$ operations are simply return
without doing anything.




The proof is easy and left to the reader.



==> sections/mutableObject.tex <==
\section{Impossibility of Emulating Mutable Objects in $M_2$}
\label{sec:mutable}

In this section we define mutable objects and show that
wait-free mutable objects cannot be simulated from SWMR
registers in $M_2$ via shared memory.
This result shows that objects like snapshot and counters, which
are simulated in $M_3$ and $M_3$ using MWMR registers
\cite{aguilera2004column,gafni2001concurrency} cannot be
implemented in systems that assume SWMR registers only. 

For a configuration $c$ and operation $a$, we denote by $c.a_i$
the sequential execution of $a$ by process $p_i$ from
configuration $c$.

Intuitively, a mutable object is one that can be changed in the
sense that a mutating operation can change the value returned by
another operation.

Formally, a \textit{Mutable object} is an object that has
operations $a$, $b$, possibly $a=b$ s.t. $\exists$ configuration
$c$ $\forall$ processes $p_i,p_j$:
$c.a_i$ returns a different value than $a_i$ in
$c.b_j.a_i$. In this case we say that $b$ $mutates$
the object.

For example, an MWMR register is a mutable object, where $a$
is a $read$ operation and $b$ is a $write(v)$ operation, and
the value of $v$ is different from the current register value.
Another example is a (possibly dynamic) atomic snapshot object,
where $a$ is a $scan$ and $b$ is an $update$.

An illustration of the proof of the following theorem can be
found in Figure \ref{fig:mutable}.


\begin{theorem}
\label{theorem:mutable}

There is no emulation of a wait-free $mutable$ object in $M_2$
from SWMR registers only.   

\end{theorem}

\begin{proof}

Assume the contrary, there is some object with operations $a$
and $b$ as in the definition of mutable objects. We construct a
sequential execution in which the mutability of the object
is contradicted.
Consider a solo execution of $a_i$ from $c$, $c.a_i$. By
wait-freedom, the operation completes and returns some value $v$,
after reading only finitely many registers. Therefore,
there is a process $p_j$ that none of its registers are read
through the execution. Now consider another execution, in which
$b_j$ executes solo from $c$ and completes in some
configuration $c'$.
In configurations $c$ and $c'$, all registers except ones
written by $p_j$ hold the same value, so a solo execution of
$a_i$ from $c'$ also completes, and the steps of $a_i$ are the
same in both executions.
Since $a$ does not read any of $p_j$'s registers the value
returned from $c.b_j.a_i$ is also $v$.
A contradiction to the assumption that $b$ mutates the object.

\end{proof}


\begin{figure}[ht]      
  \centering 
  \includegraphics[width=6in]{mutable} 
  \caption[Relations among models]
   {Theorem \ref{theorem:mutable} proof illustration:
   impossibility of wait-free mutable object emulation.}
   \label{fig:mutable}
\end{figure}

In the next section we show that by moving to dynamic models
$D_2$ and $D_3$, this result can be circumvented.

